Nonlinear Dimension Reduction via Outer Bi-Lipschitz Extensions

We introduce and study the notion of an outer bi-Lipschitz extension of a map between Euclidean spaces. The notion is a natural analogue of the notion of a Lipschitz extension of a Lipschitz map. We show that for every map $f$ there exists an outer bi-Lipschitz extension $f'$ whose distortion is greater than that of $f$ by at most a constant factor. This result can be seen as a counterpart of the classic Kirszbraun theorem for outer bi-Lipschitz extensions. We also study outer bi-Lipschitz extensions of near-isometric maps and show upper and lower bounds for them. Then, we present applications of our results to prioritized and terminal dimension reduction problems. * We prove a prioritized variant of the Johnson-Lindenstrauss lemma: given a set of points $X\subset \mathbb{R}^d$ of size $N$ and a permutation ("priority ranking") of $X$, there exists an embedding $f$ of $X$ into $\mathbb{R}^{O(\log N)}$ with distortion $O(\log \log N)$ such that the point of rank $j$ has only $O(\log^{3 + \varepsilon} j)$ non-zero coordinates - more specifically, all but the first $O(\log^{3+\varepsilon} j)$ coordinates are equal to $0$; the distortion of $f$ restricted to the first $j$ points (according to the ranking) is at most $O(\log\log j)$. The result makes a progress towards answering an open question by Elkin, Filtser, and Neiman about prioritized dimension reductions. * We prove that given a set $X$ of $N$ points in $\mathbb{R}^d$, there exists a terminal dimension reduction embedding of $\mathbb{R}^d$ into $\mathbb{R}^{d'}$, where $d' = O\left(\frac{\log N}{\varepsilon^4}\right)$, which preserves distances $\|x-y\|$ between points $x\in X$ and $y \in \mathbb{R}^{d}$, up to a multiplicative factor of $1 \pm \varepsilon$. This improves a recent result by Elkin, Filtser, and Neiman. The dimension reductions that we obtain are nonlinear, and this nonlinearity is necessary.

==> one-point.tex <==
\begin{theorem}
Let $X \subset \Rbb^d$ be a finite set of points.
Let $f \colon X \to \Rbb^{d'}$ be a function such that for every $x_1, x_2 \in X$ one has:
$$
\|f(x_1) - f(x_2)\| \in (1 \pm \eps) \cdot \|x_1 - x_2\|,
$$
where $\eps \in (0; \eps_0)$ is a (small) positive parameter. Suppose that
$x^* \in \Rbb^d \setminus X$. Then there exists $y^* \in \Rbb^{d'}$ such that
for every $x \in X$ one has:
$$
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| \in (1 \pm \delta) \cdot \|x^* - x\|,
$$
where $\delta = \eps^{\Omega(1)}$.
\end{theorem}

W.l.o.g.\ we can assume that:
\begin{itemize}
\item
The distance between $x^*$ and $X$ is equal to one;
\item
The closest to $x^*$ point from $X$ is $0$ (thus, $\|x^*\| = 1$);
\item
$f(0) = 0$.
\end{itemize}

\begin{claim}
There exists $R = \Theta(1 / \delta)$ such that if Theorem~\ref{???} is true
whenever $X \subset B(0, R)$, then it is true for any $X$.
\end{claim}
\begin{proof}
Suppose that $X \setminus B(0, R) \ne \emptyset$. Then, we invoke the theorem
for $X' = X \cap B(0, R)$ and $f$ restricted accordingly, which gives us a
point $y^* \in \Rbb^{d' + 1}$. Let us show that $y^*$ is good enough for the whole $X$
assuming $R = \Theta(1 / \delta)$ is set appropriately.

Indeed, suppose that $x \in X \setminus B(0, R)$. Then,
\begin{align*}
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| &\leq
\|f(x)\| + \|y^*\| \\&\leq  (1 + \eps)\cdot\|x\| + (1 + \delta)\cdot \|x^*\|
\\&\leq \left((1 + \eps)\cdot \frac{R}{R-1} + \frac{1+ \delta}{R-1}\right)\cdot \|x^* - x\|,
\end{align*}
where \ldots.

Similarly,
\begin{align*}
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| &\geq
\|f(x)\| - \|y^*\| \\&\geq  (1 - \eps)\cdot\|x\| - (1 + \delta)\cdot \|x^*\|
\\&\geq \left((1 - \eps)\cdot \frac{R}{R+1} - \frac{1+ \delta}{R-1}\right)\cdot \|x^* - x\|,
\end{align*}
where \ldots.

By setting $R = \Theta(1 / \delta)$ we can turn~(\ref{???}) and~(\ref{???}) into
$$
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| \leq (1 + \delta) \cdot \|x^* - x\|
$$
and
$$
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| \geq (1 - \delta) \cdot \|x^* - x\|,
$$
respectively.
\end{proof}

Thus, we can assume w.l.o.g.\ that $X \subset B(0, R)$ for $R = \Theta(1 / \delta)$.
Since the distance from $X$ to $x^*$ is equal to one, it is enough to find $y^* \in \Rbb^{d+1}$
such that for every $x \in X$ one has:
$$
\bigl\|y^* - \bigl(f(x), 0\bigr)\bigr\| \in \|x^* - x\| \pm \delta.
$$

\begin{claim}
Suppose that $x^* = \sum_{x \in X} \alpha_x \cdot x$. Let
$y^* = \sum_{x \in X} \alpha_x \cdot f(x)$. Then, for every $\widetilde{x} \in X$ one has:
$$
\bigl\|y^* - f\bigl(\widetilde{x}\bigr)\bigr\|
\in \|x^* - \widetilde{x}\| \pm O\Bigl(\sqrt{\eps} \cdot R \cdot
\bigl(1 + \|\alpha\|_1\bigr)\Bigr).
$$
\end{claim}
\begin{proof}
Define
$$
\beta_x = \begin{cases}
\alpha_x - 1, &x = \widetilde{x},\\
\alpha_x, &x \ne \widetilde{x}.\\
\end{cases}
$$
Then,
\begin{align*}
\bigl\|y^* - f\bigl(\widetilde{x}\bigr)\bigr\|^2 &
=
\Bigl\|\sum_{x \in X} \alpha_x \cdot f(x) - f\bigl(\widetilde{x}\bigr)\Bigr\|^2
\\&=
\Bigl\|\sum_{x \in X} \beta_x \cdot f(x)\Bigr\|^2
\\&=
\sum_{x_1, x_2 \in X} \beta_{x_1} \beta_{x_2} \bigl\langle f(x_1), f(x_2)\bigr\rangle
\\&=
\sum_{x_1, x_2 \in X} \frac{\beta_{x_1} \beta_{x_2}}{2} \cdot \Bigl(\bigl\|f(x_1)\bigr\|^2 + \bigl\|f(x_2)\bigr\|^2 -
\bigl\|f(x_1) - f(x_2)\bigr\|^2\Bigr)
\\&\in
\sum_{x_1, x_2 \in X} \frac{\beta_{x_1} \beta_{x_2}}{2} \cdot \Bigl(\bigl\|x_1\bigr\|^2 + \bigl\|x_2\bigr\|^2 -
\bigl\|x_1 - x_2\bigr\|^2 \pm O\bigl(\eps R^2\bigr)\Bigr)
\\&=
\sum_{x_1, x_2 \in X} \beta_{x_1} \beta_{x_2} \cdot
\Bigl(\langle x_1, x_2 \rangle\pm O\bigl(\eps R^2\bigr)\Bigr)
\\&=
\Bigl\|\sum_{x \in X} \beta_x \cdot x\Bigr\|^2 \pm O\bigl(\eps R^2 \cdot \|\beta\|_1^2\bigr)\
\\&=
\Bigl\|\sum_{x \in X} \alpha_x \cdot x - \widetilde{x}\Bigr\|^2 \pm O\bigl(\eps R^2 \cdot \|\beta\|_1^2\bigr)
\\&=
\bigl\|x^* - \widetilde{x}\bigr\|^2 \pm O\bigl(\eps R^2 \cdot \|\beta\|_1^2\bigr)
\\&\in
\bigl\|x^* - \widetilde{x}\bigr\|^2 \pm O\bigl(\eps R^2 \cdot (1 + \|\alpha\|_1)^2\bigr),
\end{align*}
where \ldots

Hence,
$$
\bigl\|y^* - f\bigl(\widetilde{x}\bigr)\bigr\| \in
\bigl\|x^* - \widetilde{x}\bigr\| \pm O\bigl(\sqrt{\eps} \cdot R \cdot (1 + \|\alpha\|_1)\bigr),
$$
since \ldots
\end{proof}

\begin{claim}
If $y^* = \|x^*\| \cdot e_{d' + 1}$, then for every $\widetilde{x} \in X$, one has:
$$
\bigl\|y^* - \bigl(f\bigl(\widetilde{x}\bigr), 0\bigr)\bigr\| \in
\bigl\|x^* - \widetilde{x}\bigr\| \pm
O
\Bigl(\max_{x \in X} \bigl|\langle x^*, x\rangle\bigr|^{1/2} + \sqrt{\eps} \cdot R\Bigr).
$$
\end{claim}

